Identity Construction in a Misogynist Incels Forum

Online communities of involuntary celibates (incels) are a prominent source of misogynist hate speech. In this paper, we use quantitative text and network analysis approaches to examine how identity groups are discussed on incels-dot-is, the largest black-pilled incels forum. We find that this community produces a wide range of novel identity terms and, while terms for women are most common, mentions of other minoritized identities are increasing. An analysis of the associations made with identity groups suggests an essentialist ideology where physical appearance, as well as gender and racial hierarchies, determine human value. We discuss implications for research into automated misogynist hate speech detection.

==> tables/cel_variants.tex <==
\begin{table}[tb]
\centering
\begin{tabularx}{\columnwidth}{X}
\toprule
\textbf{``Cel'' variants, sorted by frequency}\\
\midrule
truecels, fakecels, volcels, greycels, \\ escortcelling,
gymcelling, ricecels, mentalcels, \\ currycels, fatcels, femcels, whitecels, framecels, youngcels,
oldcels, blackcels, ethnicels, brocels, itcels, incelistan, nearcels \\
\bottomrule
\end{tabularx}
\caption{Most frequent 20 ``cel'' variants in incels.is dataset.
Plurals are combined with singular mentions and ``-ing'' terms combined with root terms. Counts range from 57,619 for ``truecels'' to 1604 for ``nearcels.''}
    \label{tab:cel_variants}
\end{table}
% Generated in cel_variants.ipynb

==> tables/cel_variants_with_counts.tex <==
\begin{table}[tbh]
\centering
\begin{tabular}{lr}
\toprule
\textbf{Term} & \textbf{Count} \\
\midrule
fakecel & 36490 \\
volcel & 35784 \\
truecel & 29301 \\
truecels & 20009 \\
fakecels & 16226 \\
ricecels & 11437 \\
greycel & 11016 \\
gymcelling & 7173 \\
trucel & 6063 \\
graycel & 6041 \\
mentalcels & 5868 \\
escortcel & 5545 \\
currycels & 5366 \\
femcels & 4901 \\
whitecels & 4745 \\
greycels & 4567 \\
youngcels & 4280 \\
escortcelling & 4190 \\
framecel & 3960 \\
escortcels & 3550 \\
fatcel & 3502 \\
\bottomrule
\end{tabular}
\caption{Most frequent ``cel'' variants in incels.is dataset. \todo{Add in more and make it ``wrapped'' and combine plural term counts, or just list them in a table for brevity and give a range in the text/full counts in an appendix.}}
    \label{tab:cel_variants}
\end{table}
% Generated in cel_variants.ipynb
